Recurrent Convolutions for Causal 3D CNNs

Recently, three dimensional (3D) convolutional neural networks (CNNs) have emerged as dominant methods to capture spatiotemporal representations in videos, by adding to pre-existing 2D CNNs a third, temporal dimension. Such 3D CNNs, however, are anti-causal (i.e., they exploit information from both the past and the future frames to produce feature representations, thus preventing their use in online settings), constrain the temporal reasoning horizon to the size of the temporal convolution kernel, and are not temporal resolution-preserving for video sequence-to-sequence modelling, as, for instance, in action detection. To address these serious limitations, here we present a new 3D CNN architecture for the causal/online processing of videos. Namely, we propose a novel Recurrent Convolutional Network (RCN), which relies on recurrence to capture the temporal context across frames at each network level. Our network decomposes 3D convolutions into (1) a 2D spatial convolution component, and (2) an additional hidden state $1\times 1$ convolution, applied across time. The hidden state at any time $t$ is assumed to depend on the hidden state at $t-1$ and on the current output of the spatial convolution component. As a result, the proposed network: (i) produces causal outputs, (ii) provides flexible temporal reasoning, (iii) preserves temporal resolution. Our experiments on the large-scale large Kinetics and MultiThumos datasets show that the proposed method performs comparably to anti-causal 3D CNNs, while being causal and using fewer parameters.

==> text/rebuttal.tex <==
\textbf{Rebuttal-561:}
\noindent
We thank the reviewers for their appreciation of the `original', `innovative' and `insightful' (in their own words) technical contribution and clear writing. Indeed, conference guidelines state that \emph{CVPR ... is looking for new ideas. We recommend that you embrace novel, brave concepts, even if they have not been tested on many datasets. ... the fact that a proposed method does not exceed the state of the art accuracy ... is not grounds for rejection}.

\textbf{Points shared among reviewers}. 
\textit{1. Absolute performance is not state-of-the-art} [51,52]. Just as gating and NL (non-local) layers provide a boost in [51,52] on top of I3D, similar layers can be applied on top of our RCN and R(2+1)D [45], as reviewers themselves acknowledge. %Since gating and NL are add on top of basic 3D
That is why we run a \emph{fair} comparison at the level of base 3D networks, i.e., RCN vs I3D and R(2+1)D [45], in the spirit of CVPR. In the same training-setup (L), RCN outperforms both I3D and R(2+1)D (Tables 2, 3, 5, and 6).

\textit{2. Low performance due to training on shorter input sequences}. 
We limited our training process to 16 frames due to lack of computational power and GPU video memory, managing to fit a batch of 64 for %I3D, RCN, and (2+1)D 
all models with input up to 16 frames. 
Any further increase in input clip length forces us to reduce batch size, leading to unstable and suboptimal training. Low batch size is already a problem with an input clip length of 8 -- a similar drop in performance is observed by the NL team\footnote{https://github.com/facebookresearch/video-nonlocal-net\#training-with-fewer-gpus} on 4 GPUs (the training process pointed out by Rev 2). The problem worsens for clip lengths 32/64.
\\
After the deadline, we managed to train our 8 frame models more efficiently, and to reproduce the results in Table 2 of [45] (absent in the current version of the paper). E.g., I3D [45] (row 2) and our trained I3D (row 4) in Table 2 now have the very same performance (61.8\%). 
At this time we are trying to improve training on 32/64 frame input clips via gradient accumulation on 4 GPUs. Achieving optimal training parameters with these computational limitations (1 4GPU machine) is challenging -- success there will encourage a host of other smaller, independent research labs (as opposed to resources-rich big tech [45,51,52]) to invest in this area. If accepted we will report all results with improved training, and make training and testing code avaible for all the models trained in this paper.
Reviewers are referred to Section 5.1 for more details on our training setup.

\textit{3. Evidence of flexible temporal reasoning} is actually discussed in Fig. 3, Sec. 6.2 (cfr. response to Rev 2).

\textit{4. Lack of FLOPs reporting:} we measured FLOPs for I3D, R(2+1)D, and RCN, recording 41MMac, 120MMac, and 54MMac, respectively. Thus, RCN requires half the FLOPs as compared to (2+1)D, and is comparable to I3D. As RCN preserves temporal resolution, it requires slightly more FLOPs than I3D. 
Remarkably, the output resolution of RCN is 8 times greater than I3D's or (2+1)D's.

\noindent
\textbf{Reviewer 3}. 
\textit{Experiments on just two datasets.}
%ECCV 2018, oral paper on causality [2] had results only on Kinetics to show causality contributions. 
We provide results on UCF101 and Kinetics (the latter a large-scale dataset), as opposed e.g. a recent ECCV oral paper [2] on causality reporting only on miniKinetics (a subset of Kinetics) dataset. 
We think this provides sufficient evidence to support our innovative idea 
in the context of fair baseline models (I3D and (2+1)D). We are working, as said, to overcome our 
resource limitations.

\noindent
\textbf{Reviewer 2} makes a number of fair points.
\textit{1. No causal tests}. Testing our model on inherently causal testbeds (e.g. online action detection) is/was actually in our plans. This could easily be a separate paper. As a first step we wanted to test absolute performance on a fair comparison basis.
Indeed we think it is unfair to compare RCN with TSN build on a better inceptionv3 base network. I3D performs better than TSN with the same base net [3]. Remarkably, RCN performs better than a anti-causal I3D, see Tables 2--6, when the base network is the same and is trained with the same setup for fair comparison. On causality, we do provide a comparison with the causal nets in [2] (Table 4) which, however, use clip length 64. The suggested causal baseline is interesting, and we will construct that in the final version.

\textit{2. No experiments temporal resolution}.
%We agree with point 
(a) The suggested solution to resolution preservation in CNNs could indeed be applicable to all the bottleneck-exploiting works, e.g. [30,32]. % or other works on image segmentation and optical flow computation.
However, [30,32] make use of deconvolution to take advantange of %the bottleneck associated with 
the decrease in resolution in convolution. %Bottleneck setup is important for 
This is crucial to these works, which is why they do not attempt to preserve resolution 
%using straight forward soultion presented 
as suggested by Rev 2. 
\\
We also agree with point (b), so we conducted an experiment in which we %unrolled RCN at test time (i.e., we 
would feed to our RCN model trained on eight frame clips an arbitrary length input video. 
We observed the same performance as in Table 2. 
I3D and (2+1)D showed instead a drop in performance, maybe because of zero padding. We pledge to report this in a final version.

\textit{3. No experiments on flexible temporal reasoning.}
GPU memory limitations is the reason we stuck to 16 frame clips. As said above, we 
will test RCN on localisation in the near future. Other 3D CNN works [51,52], nevertheless, suggest that improvements in recognition as correlated with gains in localisation as well.
Related to flexible temporal reasoning, however, we do provide in Figure 3 statistics of the weight matrices of the hidden state at every RCU layer, which suggests that the receptive field of the network increases with depth, with more focus on learning in the early stages. All this is learned implicitly by RCN. 

\iffalse
\textit{4. Low performance compared to state of the art:}
We think the training process and our GPU memory limitation is responsible for it. 
Please read the answer to common point 3.

\textit{5.} FLOPs are provided in common point 1.
\fi

\noindent
\textbf{Reviewer 1}.
\textit{1. Test videos of any length}. We observed no difference (cfr. point 2 (b) for Rev 2).

%\textit{2.} FLOPs are provided in common point 1.

\textit{3. Ablation study on different training lengths}. Although this is indeed theoretically possible for RCN, for efficiency current deep learning frameworks are based on mini batch processing, thus we could not implement this feature in PyTorch. %We will consider it in the final version if accepted. 
%However, at test time we tried on individual videos by unrolling RCN,  i.e. batch size equal to 1, see the answer to the above question.

==> text/supp_details.tex <==
In this supplementary material, 
we first present a discussion Section~\ref{sec:discus}, 
followed by implementation details in Section~\ref{subsec:details}.
Next, we show a more in-depth analysis to understand the parameters of recurrent convolution in Section~\ref{sec:more}. 

\section{Discussion}\label{sec:discus}

\subsection{Effect of Weight Initialisation.}
Weights of inflated 2D layers in ResNet (base networks)~\cite{he2016deep} 
based I3D and our RCN networks 
are initialised with weights from a pre-trained ImageNet model train on RGB images.
In the case of RCN inflation in the third dimension is 1, 
practically, it is 2D weight matrix with the third dimension being 1.
As a result, we do need to replicate the weights like in the 3D layer of I3D.

Random initialisation for hidden state parameters resulted in suboptimal training. 
Thus, in all the experiments with RCN, we used identity matrix initialisation instead.
Here we show the result of training RCN with different initilisation of 
hidden-state $w_{hh}$ convolution and spatial $w_{xh}$ convolution in Table~\ref{table:hiddenInit}.
The first row of the table where both $w_{xh}$ and $w_{hh}$ of all the RCUs in 
RCN is initialised randomly using normal initialisation process described in~\cite{he2015delving}.

Table~\ref{table:hiddenInit} show the result of different initialisation of $w_{xh}$ and $w_{hh}$ 
respectively.
It is clear from the last row of the table that RCN performs best 
if $w_{xh}$ and $w_{hh}$ are initialised with ImageNet and identity matrix respectively.
It is noteworthy that the performance difference is relatively 
small in first three rows of that table as compared to the last row jump.

\begin{table}[t]
  %\vskip -3mm
  \centering
  {\footnotesize
  %\scalebox{0.95}
  {
  \begin{tabular}{cccc}
    \toprule
    $w_{xh}$ init & $w_{hh}$ init  & Clip-Acc\% & Video-Acc\%\\ %&Vid@Avg\\ 
    \midrule
    Random & Random  & 49.0 & 61.2 \\ 
    Random & Identity  & 49.3 & 61.8 \\ 
    ImageNet & Random    & 50.4 & 62.5 \\ 
    ImageNet & Identity  & \textbf{53.0} & \textbf{65.1} \\ 
    \bottomrule
  \end{tabular}
  }
  }
  \vspace{0.1cm}
  \caption{Video-level and clip-level action recognition accuracy on 
  the Kinetics validation set for different initilisation of 2D layer ($w_{xh}$) 
  and hidden state unit weights ($w_{hh}$) in RCU with ResNet-18-based RCN models 
  trained on 8 frame-long clip as an input. 
  These results were obtained using our older training setup, 
  which was is suboptimal than the current one presented in the main paper.
  The main difference is due to data, and number iterations have increased.}
  \label{table:hiddenInit} \vspace{-1mm}
\end{table}

\subsection{ImageNet initialisation} proves to be useful for both the I3D and our RCN models.
 While (2+1)D performs (Table~\ref{table:18results}, row 6) better than RCN (row 5) 
 with the random initialisation, our RCN recovers to improve over (2+1)D (row 6) 
 with ImageNet initialisation, whereas (2+1)D cannot make use of free ImageNet initialisation.
 This seems to be a severe drawback for the (2+1)D model, and a big advantage for I3D and RCN.
 One may argue that, if the purpose is to build on existing 2D models, then RCN and I3D are a better choice, 
 whereas if new 3D models are preferred then (2+1)D might prove useful. 
 The latter does provide better performance with the random initialisation, 
 but at the price of requiring many more parameters than RCN.

% \vspace{1mm}
% \noindent
% \textbf{Random initialisation} for hidden state parameters resulted in unstable training. Thus,
% in all the experiments with RCN, we used identity matrix initialisation instead.
% Identity matrix initialisation helps to capture forget capabilities as well, 
% as suggested by~\cite{le2015simple}.
% An ablation study on the effect of initialisation is provided in the supplementary material.
%This is evident in our experiments on the very long MultiThumos videos (\S~\ref{subsec:multithumos}).

\subsection{On Input Clip Length} 
Input clip length is another factor in determining the final performance of any network. 
We can see from the Table that all the Inception-based models are trained on 64 frame-long clips, one of the reasons why Inception nets work better that ResNet models while using fewer parameters. Among the latter, ResNet101-I3D-NL~\cite{nonlocal2018wang} is shown to work better with an even longer input clip length. 
%This gain, however, comes with a tweaking of the training process -- e.g.,  Wang~\etal~\cite{nonlocal2018wang} initialise from pre-trained 32 frame-clip models and turn-off the batch normalisation layers. 
Thus, the evidence supports that training on larger input sequences boosts performance while clashing with memory limitations. 

In our experiments, as mentioned, we stuck to 8 or 16 frame clips as input and compared our proposed RCN with baseline I3D models.
We think this provides enough evidence of the validity of our proposal to move away from 
temporal convolutional networks~\cite{xie2018rethinking,nonlocal2018wang,tran2018closer,carreira2017quo}, and replace them with more sophisticated \emph{and} causal structures.
As with the role of additional layers, it is fair to predict that more extensive training on more extended clips (32,64,128) has a serious potential to take RCN to outperform state of the art in absolute terms.


\subsection{On the Efficient Training of 3D Networks}
Two basic things are clear from our experience with training heavy 3D models (I3D, (2+1)D, RCN) on large-scale datasets such as Kinetics.
Firstly, training is very computationally expensive and memory bulky; secondly, longer input clips are crucial to achieving better optimisation which, however, renders the first issue even more severe. 
We feel that how to train these model efficiently is still a wide-open problem, whose solution is essential to speed up the process for broader adoption.
We observed that ImageNet initialisation does speed up the training procedure, and helps reach local minima much quicker.
In the case of both I3D and RCN, ImageNet initialisation improves the video classification accuracy on  
Kinetics by almost $3\%$ compared to random initialisation when using the same number of training iterations, 
as shown in the first and last row of Table~\ref{table:hiddenInit}.
% Furthermore, 16 frames models also exhibit an almost $3\%$ performance improvement compared to the corresponding 8 frame models, but this comes at nearly twice the computational cost.

The bottom line is that we should strive for more efficient implementations of 3D models for the sake of their adoption. % Fabio is not that obvious?

\section{Implementation Details}\label{subsec:details}
All models with $8$ and $16$ long clip as input are trained with batch size of 
$64$ and $32$ respectively.
%and models with $16$ frame long clip are trained with batch $$
We used maximum for four 1080Ti GPUs (11GB VRAM each) while training all the models.
We used Pytorch library to implement all of the models from scratch, 
and we used the ResNet architecture of 
2D model from pytorch library's 
model zoo\footnote{https://github.com/pytorch/vision/tree/master/torchvision/models}.

\textbf{Input Data Preparations.}
We apply the same set of input data transformations to each frame in an input clip.
Data agumentation transformations include random crop, radom horizontal flip, affine transformations, and temporal jittering.


\section{Hidden State Parameters}~\label{sec:more}
Figure~\ref{fig:statsRandInits08} show the mean and 
standard deviation (Std) of weight matrixes ($w_{hh}$) 
of the hidden state at every RCU layer in our RCN network. 
We see the drop in standard deviation across different models 
(ResNet-18 in Figure~\ref{fig:statsRandInits08} and ResNet-34 in Figure~\ref{fig:statsRandInits16}(b))
 and different input clip-lengths used for training 
((8 in Figure~\ref{fig:statsRandInits08} and 16 in Figure~\ref{fig:statsRandInits16}(b))).
The drop in standard deviation and an increase in mean values of diagonal values means towards sparsity.
The increase in sparsity with depth increase can also be observed in the Figure~\ref{fig:heatmaps}, especially in the last layer (Layer 16), elements on diagonal have higher weights, and the first layer (Layer 1) has higher values distribute all around in the matrix.

We can conclude the increase in sparsity increases focuses on diagonal elements, hence, the same feature 
focus more on the time dimension of the same feature than other features from the previous hidden-state.
It is a reasonable explanation because we expect the network to learn from the different feature at small depth-level and focus more on same feature (i.e. focus on time aspect of the same feature) more with the increase in the depth-level.

\noindent
\textbf{Acknowledgement:} This work was partly supported by the European Union's Horizon 2020 research and innovation programme under grant agreement No. 779813 (SARAS).


\begin{figure*}[t]
  \centering
  \includegraphics[scale=0.50]{figures/stats-res18-s08.pdf}
  \caption{Mean and standard deviation (Std) of weight matrixes ($w_{hh}$) 
      of the hidden state at every RCU layer in the network based on ResNet-18, 
      along with the mean, and Std of diagonal elements. 
      Networks are trained on an input clip-length of 8.}
\label{fig:statsRandInits08}
\end{figure*}

\begin{figure*}[t]
  \centering
  \includegraphics[scale=0.50]{figures/s16.pdf}
  \caption{Mean and standard deviation (Std) of weight matrixes ($w_{hh}$) 
      of the hidden state at every RCU layer in the network based on ResNet-18 (a) and ResNet-34 (b), 
      along with the mean, and Std of diagonal elements. 
      Networks are trained on an input clip-length of 16.}
\label{fig:statsRandInits16}
\end{figure*}

\begin{figure*}[t]
  \centering
  \includegraphics[scale=0.5]{figures/mats.pdf}
  \caption{Heat map of weight matrixes ($w_{hh}$) 
      of the hidden state at every RCU layer in the network based on ResNet-18.
      Parula colourmap (from matlab) is used, 
      where blue is smallest values and yellow is the highest i.e. dark to bright.}
\label{fig:heatmaps}
\end{figure*}


